The LSST DESC Data Challenge 1: Generation and Analysis of Synthetic Images for Next Generation Surveys

Data Challenge 1 (DC1) is the first synthetic dataset produced by the Rubin Observatory Legacy Survey of Space and Time (LSST) Dark Energy Science Collaboration (DESC). DC1 is designed to develop and validate data reduction and analysis and to study the impact of systematic effects that will affect the LSST dataset. DC1 is comprised of $r$-band observations of 40 deg$^{2}$ to 10-year LSST depth. We present each stage of the simulation and analysis process: a) generation, by synthesizing sources from cosmological N-body simulations in individual sensor-visit images with different observing conditions; b) reduction using a development version of the LSST Science Pipelines; and c) matching to the input cosmological catalog for validation and testing. We verify that testable LSST requirements pass within the fidelity of DC1. We establish a selection procedure that produces a sufficiently clean extragalactic sample for clustering analyses and we discuss residual sample contamination, including contributions from inefficiency in star-galaxy separation and imperfect deblending. We compute the galaxy power spectrum on the simulated field and conclude that: i) survey properties have an impact of 50\% of the statistical uncertainty for the scales and models used in DC1 ii) a selection to eliminate artifacts in the catalogs is necessary to avoid biases in the measured clustering; iii) the presence of bright objects has a significant impact (2- to 6-$\sigma$) in the estimated power spectra at small scales ($\ell > 1200$), highlighting the impact of blending in studies at small angular scales in LSST;

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/DarkEnergyScienceCollaboration/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...

#main=main
main=main
default=$(shell cat .metadata.json | grep 'default_format' | cut -d'"' -f4)
outname=$(notdir $(shell pwd))

# LATEX environment variables
export TEXINPUTS:=./texmf/styles/:./tables/:
export BSTINPUTS:=./texmf/bib/:

# Files to copy when making tarball

tardir=tmp
figdir=./figures
figures=$(figdir)/*.{png,jpg,pdf}
tabdir=./tables
tables=$(tabdir)/*.tex
styles=./texmf/styles/*.{sty,cls}
bibs=./texmf/bib/*.bst
source=$(main).{tex,bbl,bib} lsstdesc.bib authors.tex acknowledgments.tex
arxiv=\def\flag{mnras}
tarfiles=$(figures) $(tables) $(styles) $(bibs) $(source)

all: export flag=\def\flag{$(default)}
all: main copy

copy:
	cp ${main}.pdf ${outname}.pdf
touch:
	touch ${main}.tex
main :
	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}

#tar : main
#	mkdir -p ${tardir}
#	cp ${tarfiles} ${tardir} | true
#	cp ${outname}.pdf ${tardir}/${outname}.pdf
#	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
#	rm -rf ${tardir}

TARGETS=aastex62 apj apjl aj prd prl mnras tex jcappub
$(TARGETS): export flag = \def\flag{$(@)}
$(TARGETS):
	$(MAKE) -e main
	$(MAKE) -e copy
	$(MAKE) -e tar
tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz



==> latexmkrc <==
# Choose which style to pass to docswitch
# NB: Default value here is always used by Overleaf
$theflag = $ENV{'STYLEFLAG'} || '\def\flag{lsstdescnote}';

# Set environment variables to search for tex inputs
# http://tex.stackexchange.com/a/50847/121099
$ENV{'TEXINPUTS'}='./desc-tex//:./tables/:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./desc-tex/bib/:' . $ENV{'BSTINPUTS'};

# Set control tools
$go_mode = 1;
$pdf_mode = 1;
# You can change the \flag value here...
$pdflatex = 'openout_any=a pdflatex %O -interaction=nonstopmode "' . $theflag . '\input{%S}"'

